RawSLAM: Online HDR Gaussian SLAM from Linear Radiance

Current dense visual SLAM systems rely almost exclusively on 8-bit tonemapped Low Dynamic Range (LDR) inputs, limiting their robustness in extreme lighting where shadows and highlights trigger tracking drift and mapping collapse. Conversely, existing raw and High Dynamic Range (HDR) reconstruction pipelines operate strictly offline. They depend on Structure-from-Motion preprocessing and are not suited for large inter-frame motion. We present, to the best of our knowledge, the first online Gaussian SLAM framework that tracks and maps directly on single-exposure 16-bit linear HDR imagery. Our method rests on three core components: an architecture-agnostic HDR Gaussian Splatting module featuring an MLP-free logarithmic parameterization of Gaussian color features; a Reinhard range-compressed photometric objective; and structure-guided spatial gradient weighting. Combined, these components allow our approach to outperform a direct HDR adaptation of MonoGS in both trajectory and reconstruction accuracy, while rendering natively in linear scene radiance for post-rendering processing. The same formulation runs unchanged on standard 8-bit inputs, roughly halving the MonoGS baseline error. Furthermore, our HDR Gaussian module transfers seamlessly to SplaTAM, Gaussian SLAM, and DROID-W, eliminating all tracking failures these systems suffer on challenging illumination sequences. To enable this research, we introduce RawSLAM: a dataset of 10 real-world indoor sequences featuring 16-bit RAW imagery, aligned depth, IMU measurements, and external OptiTrack poses. Code and dataset will be made publicly available soon.

==> sec/figures/exposure.tex <==

\begin{figure*}[t]
  \centering
  \small
  \setlength{\tabcolsep}{1pt}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{c c c c c c}
    % --- Column Titles ---
    & \textbf{0.50x} & \textbf{1.00x} & \textbf{2.00x} & \textbf{4.00x}  & \textbf{6.00x} \\%[6pt]
    
    % --- Row 1: LDR ---
    \rotatedtitle{\textbf{LDR}} &
    \griddimg{figures/exposures_candles_00141/LDR_0.5.png} &
    \griddimg{figures/exposures_candles_00141/LDR_1.0.png} &
    \griddimg{figures/exposures_candles_00141/LDR_2.0.png} &
    \griddimg{figures/exposures_candles_00141/LDR_4.0.png} &
    \griddimg{figures/exposures_candles_00141/LDR_6.0.png} & \\[-7 pt]
    % --- Row 7: HDR ---
    \rotatedtitle{\textbf{HDR}} &
    \griddimg{figures/exposures_candles_00141/HDR_0.5.png} &
    \griddimg{figures/exposures_candles_00141/HDR_1.0.png} &
    \griddimg{figures/exposures_candles_00141/HDR_2.0.png} &
    \griddimg{figures/exposures_candles_00141/HDR_4.0.png} &
    \griddimg{figures/exposures_candles_00141/HDR_6.0.png}     
  \end{tabular}
  }
  \caption{\textbf{Exposure Variation Comparison} over the resulting renders when working with LDR or HDR color spaces. Both renders were generated with our pipeline over the same scene and with the same configuration of hyperparameters. We can observe that only with HDR images we can properly apply exposure variations.}
  \label{fig:exposure_render}
\end{figure*}


%\begin{figure*}
%    \centering
%    \includegraphics[width=\linewidth]{figures/candles_00141_5exposures.png}
%    \caption{Exposure Variation Comparison over the resulting renders when using with LDR or HDR inputs. Both renders were generated with our pipeline over the same scene and with the same configuration of hyperparameters.}
%    \label{fig:exposure_render}
%\end{figure*}

==> sec/tables/LDRvsHDRinGaussianSLAM.tex <==

\begin{table}
\centering
\caption{Trajectory evaluation using ATE RMSE (cm) across different models and image formats. HDR results are obtained using log parameterization, while LDR represent the baseline. The number of fails per module is the number of scenes that diverged during training.}
\label{tab:ate_rmse_across_models}
\small % Cleaner than resizebox; scales padding naturally
\setlength{\tabcolsep}{4pt} % Tightens column padding to fit page width cleanly

\begin{tabular}{l ccccc} % Left-align first column, center data columns
\toprule
\textbf{Image Format} & \textbf{MonoGS \cite{monogs}} & \textbf{SplaTAM \cite{splatam}} & \textbf{GaussianSLAM \cite{gaussianslam}} & \textbf{Droid-W \cite{droidw}} & \textbf{ORB-SLAM 2 \cite{orbslam2}} \\ 
\midrule
Our HDR module & 39.41 & 54.26 & 57.28 & 16.46 & 4.40 \\ 
\midrule
LDR Baseline   & 56.84 & 
\begin{tabular}[c]{@{}c@{}} 89.29 \\ \scriptsize{\textbf{(3/10 FAIL)}} \end{tabular} & 
\begin{tabular}[c]{@{}c@{}} 86.93 \\ \scriptsize{\textbf{(1/10 FAIL)}} \end{tabular} & 
\begin{tabular}[c]{@{}c@{}} 16.30 \\ \scriptsize{\textbf{(1/10 FAIL)}} \end{tabular} & 
4.00 \\ 
\bottomrule \\
\end{tabular}
\end{table}


==> sec/tables/across_models_ate.tex <==
\begin{table}[t]
\centering
\caption{Mean ATE RMSE (cm) $\downarrow$ across all scenes and runs. Numbers in red superscript \textsuperscript{(\red{N})} indicate the number of scene tracking failures. The mean is computed among the succeeding runs. $^\dagger$As a sparse feature-based pipeline, ORB-SLAM2 omits the 3DGS rendering module and its "+ Our Module"  results reflect only our HDR adaptation.}
\label{tab:ate_across_models}
\footnotesize
%\setlength{\tabcolsep}{3.5pt} % Reduce ligeramente el margen horizontal entre columnas
\begin{tabularx}{0.9\linewidth}{Xccc}
\toprule
Model & \begin{tabular}[c]{@{}c@{}}Baseline\\ (LDR)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{+ Our module}\\ \textbf{(HDR)}\end{tabular} & Diff \\
\midrule
MonoGS \cite{monogs} & 53.65 & 39.41 & -14.25 \\
SplaTAM \cite{splatam} & 89.29 \textsuperscript{(\red{3})} & 54.26 & -35.03 \\
Gaussian SLAM \cite{gaussianslam} & 86.93 \textsuperscript{(\red{1})} & 57.28 & -29.65 \\
\cdashline{1-4}
\rule{0pt}{2.8ex}DROID-W \cite{droidw} & 16.30 \textsuperscript{(\red{1})} & 16.46 & + 0.16 \\
ORB-SLAM2$^\dagger$ \cite{orbslam2} & 4.00 & 4.40 & + 0.40 \\
\bottomrule
\end{tabularx}
\end{table}

==> sec/tables/across_models_per_scene.tex <==
% Requires \usepackage{multirow}, \usepackage{arydshln}, and \usepackage{colortbl} (or \usepackage[table]{xcolor})
\begin{table*}
\centering
\caption{\textbf{Metrics across SLAM frameworks per scene.} Empty skeleton table ready for data.}
\label{tab:across_models_per_scene}
\footnotesize
\renewcommand{\arraystretch}{1.2}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{ll cccccccccc}
\toprule
\multirow{2}{*}{\textbf{Scene}} & \multirow{2}{*}{\textbf{Metric}} & \multicolumn{2}{c}{\textbf{MonoGS}} & \multicolumn{2}{c}{\textbf{SplaTAM}} & \multicolumn{2}{c}{\textbf{Gaussian SLAM}} & \multicolumn{2}{c}{\textbf{Droid-W}} & \multicolumn{2}{c}{\textbf{ORB-SLAM 2}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
 &  & LDR & \cellcolor{slategray1}HDR & LDR & \cellcolor{slategray1}HDR & LDR & \cellcolor{slategray1}HDR & LDR & \cellcolor{slategray1}HDR & LDR & \cellcolor{slategray1}HDR \\
\midrule
\multirow{5}{*}{cabin} & ATE RMSE (cm) $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & SSIM $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & LPIPS $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR-$\mu$ (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
\cdashline{1-12}
\multirow{5}{*}{bottles} & ATE RMSE (cm) $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & SSIM $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & LPIPS $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR-$\mu$ (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
\cdashline{1-12}
\multirow{5}{*}{boxes} & ATE RMSE (cm) $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & SSIM $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & LPIPS $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR-$\mu$ (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
\cdashline{1-12}
\multirow{5}{*}{christmas} & ATE RMSE (cm) $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & SSIM $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & LPIPS $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR-$\mu$ (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
\cdashline{1-12}
\multirow{5}{*}{coffee} & ATE RMSE (cm) $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & SSIM $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & LPIPS $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR-$\mu$ (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
\cdashline{1-12}
\multirow{5}{*}{nerdy\_robot} & ATE RMSE (cm) $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & SSIM $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & LPIPS $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR-$\mu$ (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
\cdashline{1-12}
\multirow{5}{*}{small\_city} & ATE RMSE (cm) $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & SSIM $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & LPIPS $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR-$\mu$ (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
\cdashline{1-12}
\multirow{5}{*}{candles} & ATE RMSE (cm) $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & SSIM $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & LPIPS $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR-$\mu$ (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
\cdashline{1-12}
\multirow{5}{*}{kitchen} & ATE RMSE (cm) $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & SSIM $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & LPIPS $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR-$\mu$ (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
\cdashline{1-12}
\multirow{5}{*}{coat\_rack} & ATE RMSE (cm) $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & SSIM $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & LPIPS $\downarrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
  & PSNR-$\mu$ (dB) $\uparrow$ & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- & - & \cellcolor{slategray1}- \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> sec/tables/across_models_psnr.tex <==
\begin{table}
\centering
\caption{you should  metrics across all scenes and runs. Numbers in red superscript \textsuperscript{(\red{N})} indicate the number of scene tracking failures. The mean is computed among the succeeding runs. $^\dagger$As a sparse feature-based pipeline, ORB-SLAM2 omits our 3DGS rendering module and its "+ Our Module"  results reflect only our HDR adaptation.}
\label{tab:psnr_across_models}
\footnotesize
\renewcommand{\arraystretch}{1.1}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{tabularx}{\linewidth}{l YYY YYYY}
\toprule
& \multicolumn{3}{c}{\textbf{Baseline (LDR)}} & \multicolumn{4}{c}{\textbf{+ Our module (HDR)}} \\
\cmidrule(lr){2-4} \cmidrule(l){5-8}
\textbf{Model} 
& \begin{tabular}{@{}c@{}}{PSNR}\\(dB) $\uparrow$\end{tabular} 
& \begin{tabular}{@{}c@{}}{SSIM}\\$\uparrow$\end{tabular} 
& \begin{tabular}{@{}c@{}}{LPIPS}\\$\downarrow$\end{tabular} 
& \begin{tabular}{@{}c@{}}{PSNR}\\(dB) $\uparrow$\end{tabular} 
& \begin{tabular}{@{}c@{}}{SSIM}\\$\uparrow$\end{tabular} 
& \begin{tabular}{@{}c@{}}{LPIPS}\\$\downarrow$\end{tabular}
& \begin{tabular}{@{}c@{}}{PSNR-$\mu$}\\(dB) $\uparrow$\end{tabular}  \\
\midrule
MonoGS \cite{monogs} & 18.36 & 0.483 & 0.569 & 18.20 & 0.477 & 0.500 & 23.12 \\
SplaTAM \cite{splatam} & 19.15 & 0.708 & 0.404 & 16.76 & 0.581 & 0.5176 & 19.12 \\
Gaussian SLAM \cite{gaussianslam} & 21.44 & 0.791 & 0.400 & 19.78 & 0.720 & 0.529 & 20.68 \\
\cdashline{1-8}
\rule{0pt}{2.8ex}DROID-W \cite{droidw} & 18.87 & 0.540 & 0.528 & 16.16 & 0.426 & 0.619 & 19.95 \\
\bottomrule
\end{tabularx}
\end{table}

